Unsupervised Structure-Consistent Image-to-Image Translation

The Swapping Autoencoder achieved state-of-the-art performance in deep image manipulation and image-to-image translation. We improve this work by introducing a simple yet effective auxiliary module based on gradient reversal layers. The auxiliary module's loss forces the generator to learn to reconstruct an image with an all-zero texture code, encouraging better disentanglement between the structure and texture information. The proposed attribute-based transfer method enables refined control in style transfer while preserving structural information without using a semantic mask. To manipulate an image, we encode both the geometry of the objects and the general style of the input images into two latent codes with an additional constraint that enforces structure consistency. Moreover, due to the auxiliary loss, training time is significantly reduced. The superiority of the proposed model is demonstrated in complex domains such as satellite images where state-of-the-art are known to fail. Lastly, we show that our model improves the quality metrics for a wide range of datasets while achieving comparable results with multi-modal image generation techniques.

==> fig/ablations.tex <==
\begin{table}[!h]
\centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & LSUN Church  \\
\midrule
StyleGAN2 \cite{karras2020analyzing} & 0.377 \\
Image2StyleGAN \cite{Abdal_2019_ICCV} & 0.186 \\
Swapping \cite{DBLP:journals/corr/abs-2007-00653}& 0.227 \\
Ours & 0.203 \\

\bottomrule
\end{tabular}
% } %< \resizebox
\caption{
% 
Comparison of reconstructed image quality using LPIPS\cite{DBLP:journals/corr/abs-1801-03924} on LSUN Church. Our method focus on preserving structural details and can produce high quality results. Given the fact that our model have only been trained on 4M images which reduce the training time by a great factor, our method can reconstruct input images better than StyleGAN2 \cite{DBLP:journals/corr/abs-2007-00653}.
% 
} % \caption
\label{tab:ablations}
\end{table}

==> fig/celeba_2.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{CVPR22/fig/celeba_2.png}
\end{center}
\caption{Qualitative comparison of style transfer on CelebAMask-HQ. In each column, the first row is the texture input image and the remaining rows are the outputs according to the structure input image (first image of each row). On the second row, we can see the specular highlight on the person's face is embedded as a structure and is retained. 
 % Our model generates structure-consistent samples while transferring style from one image to another. Unlike most models that fail to preserve small structural details, our approach is able to preserve higher level of details such as earrings. 
}
\label{fig:celeba_2}
\end{figure}

==> fig/celeba_3.tex <==
\begin{figure}[!h]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=.47\textwidth]{CVPR22/fig/celeba_3.png}
\end{center}
\caption{
Illustration of style transfer on CelebAMask-HQ using our learned embedding. 
}
\label{fig:celeba_3}
\end{figure}

==> fig/celeba_5.tex <==
\begin{figure}[!ht]
% \vspace{-10pt}
\centering
\includegraphics[width=\linewidth]{CVPR22/fig/celeba_5.png}
\caption{ Additional qualitative results on CelebAMask-HQ dataset.}
\label{fig:celeba_5}
\end{figure}

==> fig/church_sup.tex <==
\begin{figure}[!t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{CVPR22/fig/church_5.png}
\end{center}
\caption{
Image translation on LSUN Church showing the quality of our method in different lightning and weather.
}
\label{fig:church_sup}
\end{figure}

==> fig/cityscapes.tex <==


%% on a $16 \times 16 \times 8$ tensor to reduce its dimension to 3. We resize the output of PCA to $256 \times 256$ for the purpose of visualization. 

==> fig/final_fig_1.tex <==
\begin{figure}
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.48\textwidth]{CVPR22/fig/celeba_nice.png}
% \hfill
% \includegraphics[width=.99\columnwidth]{CVPR22/fig/church_interesting_results.png}

\end{center}
\caption{
% 
% Left: Results from Swapping Autoencoder \cite{DBLP:journals/corr/abs-2007-00653} on LSUN Church. Right: Our results on the same images. As evident, our model achieves better feature embedding and can retain the structural information of the input image while swapping only the texture with that of a second input image. Finer-level details such as spires and buildings outline are also retained. Most notably, our model was trained for a fraction of iterations compared to \cite{DBLP:journals/corr/abs-2007-00653}.
}
\label{fig:final_supp_1}
\end{figure}

==> fig/final_fig_2.tex <==
\begin{figure}
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
% \includegraphics[width=.99\columnwidth]{CVPR22/fig/celeba_nice.png}
% \hfill
\includegraphics[width=.47\textwidth]{CVPR22/fig/church_interesting_results.png}

\end{center}
\caption{
Illustration of some limitations of our method. Top right shows the learned structure embedding.
% 
% Left: Results from Swapping Autoencoder \cite{DBLP:journals/corr/abs-2007-00653} on LSUN Church. Right: Our results on the same images. As evident, our model achieves better feature embedding and can retain the structural information of the input image while swapping only the texture with that of a second input image. Finer-level details such as spires and buildings outline are also retained. Most notably, our model was trained for a fraction of iterations compared to \cite{DBLP:journals/corr/abs-2007-00653}.
}
\label{fig:final_supp_2}
\end{figure}

==> fig/inria.tex <==
\begin{figure}[!ht]
\includegraphics[width=0.47\textwidth]{CVPR22/fig/inria.png}
\caption{
\textbf{Performance on Inria dataset.} Left-to-right: first input $x_1$, second input $x_2$, reconstruction of $x_1$, our generated sample using structure of $x_1$ and texture of $x_2$.
The first column shows the structure reference images, the second column the texture reference images from which we extract their texture embedding. The third column shows the reconstructions of the first column using the learnt latent codes. The last column shows the synthesized images with the style transferred from the second image while preserving the structure of the first.
Learning consistent embedding for aerial imagery is clearly more complex than single object datasets. We argue that given the complexity of the problem our method still preserves fine details such as front and back windows of the cars which shows its potential.
% \todo{final goal is to have a detailed analysis of the challenges, where it fails and why it's a worthwhile task. I can also talk about the details of generated samples like the windows on small cars}
}
\label{fig:inria}
\end{figure}

==> fig/sota_v2._validation.tex <==
\begin{table}[!h]
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & LSUN Church & CelebAMask-HQ & Cityscapes  \\
\midrule
Ours & 52.96$\pm$1.7 & 29.69 & 174.8 \\
Swapping \cite{DBLP:journals/corr/abs-2007-00653} & 52.34 & 32.83 & 182.5 \\
StyleGAN2 \cite{karras2020analyzing} & 57.54 & - & - \\
MaskGAN \cite{CelebAMask-HQ} & - & 46.84 & -\\
SMIS \cite{DBLP:journals/corr/abs-2003-12697} & - & - & 49.81 \\ 
BicycleGAN \cite{DBLP:journals/corr/abs-1711-11586} & - & - & 87.74\\



\bottomrule
\end{tabular}
} % \resizebox
\caption{
Quantitative comparison of FID on style transfer with some label-to-image translation work that are known for multimodal image synthesis and Swapping Autoencoder. In cases that we didn't have access to metric values calculated by the author, we trained their model for the same number of iterations as our network. Our method can achieve better results on CelebAMask-HQ and comparable results on LSUN Church trained for only 1.2M and 4M images. 
% 
} % \caption
\label{tab:sota_v2_validataion}
\end{table}


% Inria ours: 191.53
% Inria Swapping: 

==> fig/supplementary_1.tex <==
\begin{figure*}
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{CVPR22/fig/inria_road.png}

\end{center}
\caption{
This figure provide an example of how our method can preserve the geometry of objects and semantic details while transferring the style. This would allow us to generate multiple samples with no extra labeling cost.
}
\label{fig:inria_road}
\end{figure*}

==> fig/supplementary_2.tex <==
\begin{figure}
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{CVPR22/fig/celeba_4.png}
% \vfill
% \includegraphics[width=\textwidth]{}

\end{center}
\caption{
The first(left) image shows the first input image, and the second/third/fourth images show the generated image where the structure is retained from the first input image and the texture from the second/third/fourth input image, which appear in the inset images.}
\label{fig:celeba_sup}
\end{figure}
